Acoustic detection of astrophysical neutrinos in South Pole ice

When high-energy particles interact in dense media to produce a particle shower, most of the shower energy is deposited in the medium as heat. This causes the medium to expand locally and emit a shock wave with a medium-dependent peak frequency on the order of 10 kHz. In South Pole ice in particular, the elastic properties of the medium have been theorized to provide good coupling of particle energy to acoustic energy. The acoustic attenuation length has been theorized to be several km, which could enable a sparsely instrumented large-volume detector to search for rare signals from high-energy astrophysical neutrinos. We simulated a hybrid optical/radio/acoustic extension to the IceCube array, specifically intended to detect cosmogenic (GZK) neutrinos with multiple methods simultaneously in order to achieve high confidence in a discovered signal and to measure angular, temporal, and spectral distributions of GZK neutrinos. This work motivated the design, deployment, and operation of the South Pole Acoustic Test Setup (SPATS). The main purpose of SPATS is to measure the acoustic attenuation length, sound speed profile, noise floor, and transient noise sources \emph{in situ} at the South Pole. We describe the design, performance, and results from SPATS. We measured the sound speed in the fully dense ice between 200 m and 500 m depth to be 3878 $\pm$ 12 m/s for pressure waves and 1975.8 $\pm$ 8.0 m/s for shear waves. We measured the acoustic amplitude attenuation length to be 316 $\pm$ 105 m. We measured the background noise floor to be Gaussian and very stable on all time scales from one second to two years. Finally, we have detected an interesting set of well-reconstructed transient events in over one year of high quality transient data acquisition. We conclude with a discussion of what is next for SPATS and of the prospects for acoustic neutrino detection in ice.

==> 00README.XXX.tex <==
vandenbroucke_thesis.tex toplevelfile
